SEAGLE: A Scalable Exact Algorithm for Large-Scale Set-Based GxE Tests in Biobank Data

The explosion of biobank data offers immediate opportunities for gene-environment (GxE) interaction studies of complex diseases because of the large sample sizes and the rich collection in genetic and non-genetic information. However, the extremely large sample size also introduces new computational challenges in GxE assessment, especially for set-based GxE variance component (VC) tests, which are a widely used strategy to boost overall GxE signals and to evaluate the joint GxE effect of multiple variants from a biologically meaningful unit (e.g., gene). In this work, we focus on continuous traits and present SEAGLE, a Scalable Exact AlGorithm for Large-scale set-based GxE tests, to permit GxE VC tests for biobank-scale data. SEAGLE employs modern matrix computations to achieve the same "exact" results as the original GxE VC tests without imposing additional assumptions or relying on approximations. SEAGLE can easily accommodate sample sizes in the order of $10^5$, is implementable on standard laptops, and does not require specialized computing equipment. We demonstrate SEAGLE's performance through extensive simulations. We illustrate its utility by conducting genome-wide gene-based GxE analysis on the Taiwan Biobank data to explore the interaction of gene and physical activity status on body mass index.

==> app2.tex <==
\section{Appendix: Restricted Maximum Likelihood (REML) EM Algorithm for Estimating Variance Components}
\label{app:em-reml}

Under the null hypothesis $H_0:\nu=0$ and the assumptions that $\tau> 0$ and $\sigma> 0$, model \eqref{eqn:mixedmodel} becomes
\begin{eqnarray}\label{eqn:nullmodel}
\vy &=& \mtx\vbeta + \mg\vb + \veps,
\end{eqnarray}
where $\vb \sim \text{N}({\bf 0}, \tau \,\mi_{L})$ and $\veps\sim \text{N}(\vzero, \sigma\,\mi_{n})$ are uncorrelated.  Assume that $\mtx$ has full column rank so that $\rank(\mtx) = P$.  Let $\vu = \ma\Tra\vy$ %be a set of $n-P$ linearly independent contrasts 
such that $\ma\ma\Tra = \mi - \mtx(\mtx\Tra\mtx)\Inv\mtx\Tra$ and $\ma\Tra\ma = \mi_{n-P}$.  Then 
\begin{eqnarray*}
	\vu &=& \ma\Tra \vy \\
		&=& \ma\Tra\mg\vb + \ma\Tra\veps
\end{eqnarray*}
so that $\vu \given \vb$ does not depend on the unobserved fixed effects parameter $\vbeta$.

Following the work in \citep{tzeng2011studying},   
we consider an expectation-maximization (EM) algorithm based on the restricted maximum likelihood for the observed data $\vu$ and missing data $\vb$ 
with the following complete data log likelihood
\begin{eqnarray}\label{eqn:emloglikelihood}
	\log f(\vu, \vb; \tau, \sigma) 
		&=& \log f(\vu \given \vb ; \tau, \sigma) + \log f(\vb ; \tau, \sigma).
\end{eqnarray}
For the first term on the right-hand side of \eqref{eqn:emloglikelihood}, we use the fact that the conditional distribution of $\vu$ given $\vb$ is
\begin{eqnarray*}
	\vu \given \vb \sim \text{N}(\ma\Tra\mg\vb, \sigma\,\mi_{n-P})
\end{eqnarray*}
so that 
\begin{eqnarray*}
	f(\vu \given \vb; \tau, \sigma) &=& (2\pi)^{-\frac{n-P}{2}} \, |\sigma\,\mi_{n-P}|^{-\frac{1}{2}} \, \exp\left\{-\frac{1}{2\sigma}\|\vu - \ma\Tra\mg\vb\|^{2}_{2}\right\}
\end{eqnarray*}
and
\begin{eqnarray}\label{eqn:logf_ygivenb}
	\log f(\vu \given \vb; \tau, \sigma) &\propto& -\frac{n-P}{2}\,\log \sigma 	
		-\frac{1}{2\sigma}\|\vu - \ma\Tra\mg\vb\|^{2}_{2}.
\end{eqnarray}
For the second term on the right-hand side of \eqref{eqn:emloglikelihood}, we have
\begin{eqnarray*}
	f(\vb ; \tau, \sigma) &=& (2\pi)^{-\frac{L}{2}} \, |\tau\,\mi_{L}|^{-\frac{1}{2}} \, \exp\left\{ -\frac{1}{2\tau} \|\vb\|^{2}_{2} \right\}
\end{eqnarray*}
so that
\begin{eqnarray}\label{eqn:logf_b}
	\log f(\vb; \tau, \sigma) &\propto& -\frac{L}{2} \log \tau - \frac{1}{2\tau} \|\vb\|^{2}_{2}.
\end{eqnarray}
Inserting \eqref{eqn:logf_ygivenb} and \eqref{eqn:logf_b} into \eqref{eqn:emloglikelihood} gives
\begin{eqnarray*}
	\log f(\vu, \vb; \tau, \sigma) 
	&\propto&
		-\frac{n-P}{2}\,\log \sigma  	
		-\frac{1}{2\sigma}\|\vu - \ma\Tra\mg\vb\|^{2}_{2} 
		-\frac{L}{2} \log \tau - \frac{1}{2\tau} \|\vb\|^{2}_{2}.
\end{eqnarray*}
Therefore, $Q(\tau, \sigma; \tauhatt, \sigmahatt)$ in the expectation step (E-step) is
\begin{eqnarray*}
	Q(\tau, \sigma; \tauhatt, \sigmahatt) &\equiv&	
		\Exp\left[ \log f(\vu, \vb; \tau, \sigma) \given \vu; \tauhatt, \sigmahatt \right] \\
		&\propto& -\frac{n-P}{2} \log \sigma - \frac{1}{2\sigma} \, \Exp\left[ \|\vu - \ma\Tra\mg\vb\|^{2}_{2} \given \vu; \tauhatt, \sigmahatt \right] \\
		&\;\;\;\;\;& 
		- \frac{L}{2}\log \tau - \frac{1}{2\tau}\, \Exp\left[ \|\vb\|^{2}_{2} \given \vu; \tauhatt, \sigmahatt \right].
\end{eqnarray*}

To obtain the distribution of $\vb \given \vu$, we recall the fact that for any $\vg_{1} \in \mathbb{R}^{q}$ and $\vg_{2} \in \mathbb{R}^{N-q}$ such that
\begin{eqnarray*}
	\begin{bmatrix} \vg_{1} \\ \vg_{2} \end{bmatrix} \sim
	\text{N}\left( \begin{bmatrix}\vmu_{1} \\ \vmu_{2}\end{bmatrix}, \begin{bmatrix} \Sigma_{11} & \Sigma_{12} \\ \Sigma_{21} & \Sigma_{22} \end{bmatrix} \right),
\end{eqnarray*}
the distribution of $\vg_{1} \given \vg_{2}$ is
\begin{eqnarray*}
	\vg_{1} \given \vg_{2} \sim \text{N}(\vmu_{1} + \Sigma_{12}\Sigma_{22}\Inv(\vg_{2}-\vmu_{2}), \Sigma_{11}-\Sigma_{12}\Sigma_{22}\Inv\Sigma_{21}).
\end{eqnarray*}
Since the covariance between $\vb$ and $\vu$ is
\begin{eqnarray*}
	\Cov(\vb, \vu) &=& \Exp[\vb(\vu-\Exp[\vu])\Tra] \\
		&=& \Exp[\vb\{\ma\Tra(\mtx\vbeta + \mg\vb + \veps) - \vzero\}\Tra] \\%- \vzero \\
		&=& \Exp[\vb\,\vb\Tra\mg\Tra\ma] \\
		&=& \Var(\vb)\mg\Tra\ma = \tau\,\mg\Tra\ma = \Sigma_{12},
\end{eqnarray*}
the joint distribution of $\vb$ and $\vu$ is
\begin{eqnarray*}
	\begin{bmatrix} \vb \\ \vu \end{bmatrix} \sim \text{N}\left(
		\begin{bmatrix} \vzero \\ \vzero \end{bmatrix}, 
		\begin{bmatrix} \tau \, \mi_{L} & \tau \,\mg\Tra\ma \\
					\tau\,\ma\Tra\mg & \tau\,\ma\Tra\mk_{G}\ma + \sigma\,\mi_{n-P} \end{bmatrix}
	 \right)
\end{eqnarray*}
and we have
\begin{eqnarray*}
	\vb\given \vu \sim \text{N}(\tau\,\mg\Tra\ma\mr\Inv\vu, \tau\,\mi_{L}-\tau^{2}\,\mg\Tra\ma\mr\Inv\ma\Tra\mg),
\end{eqnarray*}
where $\mr = \tau\,\ma\Tra\mk_{G}\ma+\sigma\,\mi_{n-P}$.  Therefore, in the maximization step (M-step), we have 
\begin{eqnarray*}
	\frac{\partial Q}{\partial \sigma} &=& -\frac{n-P}{2\sigma} + \frac{1}{2\sigma^{2}} \Exp\left[ \| \vu-\ma\Tra\mg\vb\|^{2}_{2} \given \vu; \tauhatt, \sigmahatt \right]
\end{eqnarray*}
so that
\begin{eqnarray*}%\label{eqn:sigmaupdate}
	\sigmahattp &=& \frac{1}{n-P} \Exp\left[ \| \vu-\ma\Tra\mg\vb\|^{2}_{2} \given \vu; \tauhatt, \sigmahatt \right] \nonumber \\
	&=& \frac{1}{n-P} \left[ \|\vu - \tauhatt\,\ma\Tra\mk_{G}\ma\mr\Inv\vu\|^{2}_{2} + \tauhatt\,\trace(\ma\Tra\mk_{G}\ma-\tauhatt\, \ma\Tra\mk_{G}\ma\mr\Inv\ma\Tra\mk_{G}\ma) \right]
\end{eqnarray*}
since $\Exp[\vu-\ma\Tra\mg\vb \given \vu] = \vu - \tau\ma\Tra\mk_{G}\ma\mr\Inv\vu$ and $\Var(\vu-\ma\Tra\mg\vb\given\vu)=\tau\,\ma\Tra\mk_{G}\Tra\ma - \tau^2\ma\Tra\mk_{G}\ma\mr\Inv\ma\Tra\mk_{G}\ma$.  For the first term on the right, we have
\begin{eqnarray*}
	\vu - \tauhatt \, \ma\Tra\mk_{G}\ma\mr\Inv\vu 
		&=& (\mr\mr\Inv - \tauhatt \, \ma\Tra\mk_{G}\ma\mr\Inv)\vu \\
		&=& (\mr - \tauhatt \, \ma\Tra\mk_{G}\ma)\mr\Inv\vu \\
		&=& \sigmahatt \,\mr\Inv\vu.
\end{eqnarray*}
For the second term on the right, we have
\begin{eqnarray*}
	\tauhatt\,\trace(\ma\Tra\mk_{G}\ma-\tauhatt\, \ma\Tra\mk_{G}\ma\mr\Inv\ma\Tra\mk_{G}\ma)
	&=& \trace\left([\mr - \tauhatt\, \ma\Tra\mk_{G}\ma]\tauhatt\,\mr\Inv\ma\Tra\mk_{G}\ma \right) \\
	&=& \sigmahatt \,\tauhatt\,\trace(\mr\Inv\ma\Tra\mk_{G}\ma) \\
	&=& \sigmahatt\, \tauhatt\, \trace(\mg\Tra\ma\mr\Inv\ma\Tra\mg).
\end{eqnarray*}
Inserting these simplifications into the update for $\sigmahatt$ gives us
\begin{eqnarray}\label{eqn:sigmaupdate}
	\sigmahattp &=& \frac{1}{n-P} \left[ \|\sigmahatt \,\mhr\Inv\vu\|^{2}_{2} + \sigmahatt\,\tauhatt\,\trace(\mg\Tra\ma\mhr\Inv\ma\Tra\mg) \right], 
\end{eqnarray}
where $\mhr = \tauhatt\, \ma\Tra\mk_{G}\ma + \sigmahatt\, \mi_{n-P}$.

Additionally, we have
\begin{eqnarray*}
	\frac{\partial Q}{\partial \tau} &=& -\frac{L}{2\tau} + \frac{1}{2\tau^{2}}\Exp[\|\vb\|^{2}_{2} \given \vu; \tauhatt, \sigmahatt]
\end{eqnarray*}
so that
\begin{eqnarray}\label{eqn:tauupdate}
	\tauhattp &=& \frac{1}{L}\Exp[\|\vb\|^{2}_{2} \given \vu; \tauhatt, \sigmahatt] \nonumber\\
		&=& \frac{1}{L}\left[ \tauhatt^{2}\, \|\mg\Tra\ma\mhr\Inv\vu\|^{2}_{2} + \text{tr}(\tauhatt\,\mi_{L}-\tauhatt^{2}\mg\Tra\ma\mhr\Inv\ma\Tra\mg) \right].
\end{eqnarray}



==> appFigTab.tex <==
\section{Supplementary Tables and Figures}
\label{sec:suppl_tab_fig}

%%%%%%%%%%%%%%%%%

\begin{figure}[H]
\begin{center}
\includegraphics[width=0.5\textwidth]{figureS1}
\end{center}
\caption{\emph{Quantile-Quantile plot depicting p-values over $N=1{,}000$ replicates for $n=5{,}000$ observations and $L=100$ loci under the null hypothesis in the random effects simulations.}}
\label{fig:sim1a_qq}
\end{figure}
%%%%%%%%%%%%%%%%%

\begin{figure}
%\begin{minipage}{0.48\textwidth}
%\centering
%\captionsetup{type=table} %% tell latex to change to table
%\begin{tabular}{lr}\hline
%      & MSE of p-value  \\ \hline
%SEAGLE &        $3.49\times 10^{-4}$          \\
%MAGEE & $224.96\times 10^{-4}$          \\
%OVC & $3.49\times 10^{-4}$          \\
%FastKM & $17.88\times 10^{-4}$          \\\hline
%\end{tabular}
%\begin{center}(A) \end{center}
%%\caption{\emph{Mean square error (MSE) of the p-values obtained from different GxE VC test, compared to the "truth" p-values. }}
%\label{tab:mse_pv}
%\end{minipage}
%\begin{minipage}{0.48\textwidth}
\centering
\includegraphics[width=0.5\textwidth]{figure2}
%\begin{center}(B) \end{center}
%\caption{\emph{Absolute relative error from p-value obtained with true $\tau=1$ and $\sigma=1$ values over $N=1{,}000$ replicates with $n=5{,}000$ observations and $L=100$ loci.}}\label{fig:sim1a_relerror}
%\end{minipage}
\caption{\emph{Absolute relative error of the p-values obtained from different GxE VC tests, compared to the ``Truth" p-values. Results are obtained with $\tau=\sigma=1$ under $H_0:\nu=0$ over $N=1{,}000$ replicates with $n=5{,}000$ observations and $L=100$ loci.}}
\label{fig:mse_re_pv}
\end{figure}


%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
	\begin{center}
		\includegraphics[width=\textwidth]{figureS2}
	\end{center}
	\caption{\emph{Quantile-quantile plots for p-values obtained over $N=1{,}000$ replicates for $n=20{,}000$ and $n=100{,}000$ observations and $L=100$ loci  in the fixed effects simulations.}}
	\label{fig:sim2a_qq}
\end{figure}

%%%%%%%%%%%%%%%%%
\begin{figure}[H]
	\begin{center}
		\includegraphics[width=\textwidth]{figureS3}
	\end{center}
	\caption{\emph{Estimated values for $\tau$ and $\sigma$ over $N=1{,}000$ replicates with $n=20{,}000$ observations and $L=100$ loci.}}
	\label{fig:sim2a_varcomps}
\end{figure}


%%%%%%%%%%%%%%%%%
\begin{table}[H]
	\caption{\emph{P-values of the G$\times$PA effects (i.e., interactions between genes and physical activity (PA)) on body mass index (BMI), identified by SEAGLE and MAGEE in the Taiwan Biobank study at the $5\times 10^{-4}$ nominal level. Relevance scores are obtained from GeneCards human gene database (www.genecards.org) using multiword search with string "'body mass index' OR obesity OR 'physical activity'".}}
	\label{table:twb_bmi}
\begin{center}
\begin{tabular}{cccc}\hline
\multirow{2}{*}{Gene} & \multirow{2}{*}{SEAGLE} & \multirow{2}{*}{MAGEE} & Relevance Score with\\
&&& BMI, obesity or PA \\ \hline
%Gene      & SEAGLE   & MAGEE    & Relevance Scores with BMI/obesity/PA \\ \hline
ALOX5AP   & 4.33E-04 & -        & 6.16                                              \\
BCLAF1    & 1.83E-04 & -        & 0.26                                              \\
CBLN2     & 3.05E-05 & 3.71E-05 & -                                                 \\
FCN2      & 4.08E-04 & 2.70E-04 & 0.56                                              \\
FOXR1     & 3.22E-04 & 1.53E-04 & -                                                 \\
LOC338694 & 1.34E-04 & 1.83E-04 & -                                                 \\
OCM       & 4.18E-04 & 8.58E-05 & 0.91                                              \\
PCDH17    & 3.64E-04 & -        & 1.54                                              \\
TBPL1     & -        & 2.24E-04 & - \\ \hline                              
\end{tabular}
\end{center}
\end{table}

